Large Language Models for Compiler Optimization

We explore the novel application of Large Language Models to code optimization. We present a 7B-parameter transformer model trained from scratch to optimize LLVM assembly for code size. The model takes as input unoptimized assembly and outputs a list of compiler options to best optimize the program. Crucially, during training, we ask the model to predict the instruction counts before and after optimization, and the optimized code itself. These auxiliary learning tasks significantly improve the optimization performance of the model and improve the model's depth of understanding. We evaluate on a large suite of test programs. Our approach achieves a 3.0% improvement in reducing instruction counts over the compiler, outperforming two state-of-the-art baselines that require thousands of compilations. Furthermore, the model shows surprisingly strong code reasoning abilities, generating compilable code 91% of the time and perfectly emulating the output of the compiler 70% of the time.

==> acknowledgements.tex <==
% Mike Lewis, Baptiste, Armen, et al.

==> listings/ir-normalization.tex <==
\begin{figure}
\setcaptiontype{lstlisting}
\begin{minipage}[]{1\columnwidth}
    \begin{lstlisting}[language=LLVM]
define dso_local i32 @fib(i32 %0) #0 {
  br label %2

2:                                      ; preds = %6, %1
  %3 = phi i32 [ 1, %1 ], [ %8, %6 ]
  %4 = phi i32 [ %0, %1 ], [ %7, %6 ]
  %5 = icmp eq i32 %4, 0
  br i1 %5, label %9, label %6

6:                                      ; preds = %2
  %7 = add nsw i32 %4, -1
  %8 = mul nsw i32 %4, %3
  br label %2

9:                                      ; preds = %2
  ret i32 %3
}
    \end{lstlisting}
    \subcaption{Before.}
\end{minipage}
\begin{minipage}[]{1\columnwidth}
    \begin{lstlisting}[language=LLVM]
define dso_local i32 @"fib"(i32 %0) {
br label %2

2:
%3 = phi i32 [1, %1], [%8, %6]
%4 = phi i32 [%0, %1], [%7, %6]
%5 = icmp eq i32 %4, 0
br i1 %5, label %9, label %6

6:
%7 = add nsw i32 %4, 1
%8 = mul nsw i32 %4, %3
br label %2

9:
ret i32 %3
}
    \end{lstlisting}
    \subcaption{After.}
\end{minipage}
\caption{Normalizing LLVM-IR.}
\label{listings/codegen-type-errors}
\end{figure}


==> tables/bpe.tex <==
\begin{table}
  \caption{%
  Comparison of vocabularies on a holdout set of 1k LLVM-IR functions. Llama 32k and LLVM 32k both split on whitespace and digits. We then trained a further vocabulary with only splitting on newlines. The LLVM vocabularies were trained on 1B characters of (Prompt, Answer) pairs from the training corpus. \todo{HJL: If only from scratch model, don't need all rows? Is row 2 needed?} \todo[Chris]{Column to show word splitting strategy}
}
  \scriptsize
  \label{tables/bpe}
  \centering
  \begin{tabular}{lccc}
    \toprule
    & $n$ tokens & chars per token & compression \\
    \midrule
    Llama~\cite{llama} & 823,870 & 2.024 & 1.00$\times$ \\
    LLVM & 635,827 & 2.622 & 1.30$\times$  \\
    LLVM line-level & 246,471 & 6.764 & 3.34$\times$  \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/model-architectures.tex <==
\begin{table}
  \caption{Model architectures. Training time is wall time measurement on single node with 8$\times$ NVIDIA V100s. \todo{cummins}{Names \& results are placeholders}}
  \label{tables:model-architectures}
  \centering
  \begin{tabular}{cR{1.5cm}R{1.5cm}cC{1.5cm}c}
    \toprule
    params     & $n$ heads & $n$ layers & dimension & sequence length & GPU-hours \\
    \midrule
    135M & 12 & 12 & 768 & 1024 & 7 days\\  % Tessar1
    135M & 12 & 12 & 768 & 512 & 5 days\\   % Bio1
    370M & 16 & 24 & 1024 & 1024 & 21 days\\  % Tessar3
    370M & 16 & 24 & 1024 & 512 & 17 days\\  % Bio3
    \bottomrule
  \end{tabular}
\end{table}

